Beyond Visual Similarity: Rule-Guided Multimodal Clustering with explicit domain rules

Traditional clustering techniques often rely solely on similarity in the input data, limiting their ability to capture structural or semantic constraints that are critical in many domains. We introduce the Domain Aware Rule Triggered Variational Autoencoder (DARTVAE), a rule guided multimodal clustering framework that incorporates domain specific constraints directly into the representation learning process. DARTVAE extends the VAE architecture by embedding explicit rules, semantic representations, and data driven features into a unified latent space, while enforcing constraint compliance through rule consistency and violation penalties in the loss function. Unlike conventional clustering methods that rely only on visual similarity or apply rules as post hoc filters, DARTVAE treats rules as first class learning signals. The rules are generated by LLMs, structured into knowledge graphs, and enforced through a loss function combining reconstruction, KL divergence, consistency, and violation penalties. Experiments on aircraft and automotive datasets demonstrate that rule guided clustering produces more operationally meaningful and interpretable clusters for example, isolating UAVs, unifying stealth aircraft, or separating SUVs from sedans while improving traditional clustering metrics. However, the framework faces challenges: LLM generated rules may hallucinate or conflict, excessive rules risk overfitting, and scaling to complex domains increases computational and consistency difficulties. By combining rule encodings with learned representations, DARTVAE achieves more meaningful and consistent clustering outcomes than purely data driven models, highlighting the utility of constraint guided multimodal clustering for complex, knowledge intensive settings.

==> sec/de.tex <==
\begin{table}
\centering
\caption{Automotive hard clustering (K-means) performance comparison}
\label{tab:automotive_clustering}
\begin{tabular}{cccc}
\hline
Config& SS & DB & CH \\
\hline
Baseline      & 0.054 & 3.271 & 173.8 \\
Rule-Guided   & 0.139 & 0.924 & 12234.9 \\
\hline
\multicolumn{4}{l}{\textbf{Rule Violations (Rule-Guided)}} \\
Body          & 3.01   &        &         \\
Performance   & 4.83   &        &         \\
Size          & 3.92   &        &         \\
Luxury        & 4.53   &        &         \\
\hline
\multicolumn{4}{l}{\footnotesize Total violations: Baseline = 0,
Rule-Guided = 16.29} \\
%\multicolumn{4}{l}{\footnotesize SS: Silhouette Score, DB: Davies-Bouldin Score, 
%CH: Calinski-Harabasz Score}
\end{tabular}
\end{table}
\begin{table*}
\centering
\caption{Automotive soft clustering (Fuzzy C-means) performance comparison}
\label{tab:automotive_fuzzy}
\begin{tabular}{lcccc}
\hline
Configuration & FPC & FPE & MS & FS \\
\hline
Baseline    & 0.1250 & 2.0794 & 0.1250 & 0.1679 \\
Rule-Guided & 0.1250 & 2.0794 & 0.1250 & 0.1897 \\
Improvement & 0\%    & 0\%    & 0\%    & 13.0\% \\
\hline
\multicolumn{5}{l}{\textbf{Rule Violations (Rule-Guided)}} \\
Body        & 0.19  &       &       &      \\
Performance & 3.60  &       &       &      \\
Size        & 2.00  &       &       &      \\
Luxury      & 2.72  &       &       &      \\
\hline
\multicolumn{5}{l}{\footnotesize Total violations: Baseline = 0, Rule-Guided = 8.51} \\
\multicolumn{5}{l}{\footnotesize FPC: Fuzzy Partition Coefficient, FPE: Fuzzy Partition Entropy,} \\
\multicolumn{5}{l}{\footnotesize MS: Average Membership Strength, FS: Fuzzy Silhouette Index}
\end{tabular}
\end{table*}

\begin{table*}
\centering
\caption{Aircraft hard clustering (K-means) performance across rule configurations}

\label{tab:aircraft_clustering}
\begin{tabular}{l|ccc|cccc}
\hline
\multirow{2}{*}{Configuration} & \multicolumn{3}{c|}{Hard Clustering Metrics} & \multicolumn{4}{c}{Rule Violations} \\
& SS & DB & CH & Stealth & UAV & Mission & Semantic \\
\hline
Baseline & 0.1406 & 1.5167 & 174.37 & -- & -- & -- & -- \\
2-Rule & 0.7109 & 1.0666 & 16,325.64 & 85 & 0 & -- & -- \\
4-Rule & 0.3325 & 0.9147 & 794.43 & 85 & 0 & 401 & 103 \\
\hline
\multicolumn{8}{l}{\footnotesize SS: Silhouette Score, DB: Davies-Bouldin Score, CH: Calinski-Harabasz Score}
\end{tabular}
\end{table*}
\begin{table*}
\centering
\caption{Automotive soft clustering (Fuzzy C-means) performance comparison}
\label{tab:automotive_fuzzy}
\begin{tabular}{l|cccc|cccc}
\hline
\multirow{2}{*}{Configuration} & \multicolumn{4}{c|}{Fuzzy Clustering Metrics} & \multicolumn{4}{c}{Rule Violations} \\
& FPC & FPE & MS & FS & Body & Performance & Size & Luxury \\
\hline
Baseline & 0.1250 & 2.0794 & 0.1250 & 0.1679 & -- & -- & -- & -- \\
Rule-Guided & 0.1250 & 2.0794 & 0.1250 & 0.1897 & 0.19 & 3.60 & 2.00 & 2.72 \\
Improvement & 0\% & 0\% & 0\% & 13.0\% & -- & -- & -- & -- \\
\hline
\multicolumn{9}{l}{\footnotesize Total violations: Baseline = 0, Rule-Guided = 8.51} \\
\multicolumn{9}{l}{\footnotesize FPC: Fuzzy Partition Coefficient, FPE: Fuzzy Partition Entropy,} \\
\multicolumn{9}{l}{\footnotesize MS: Average Membership Strength, FS: Fuzzy Silhouette Index}
\end{tabular}
\end{table*}

%--------------------------------------------------------------------------------

\begin{table*}
\centering
\caption{Aircraft soft clustering (Fuzzy C-means) performance across rule configurations}
\label{tab:aircraft_fuzzy}
\begin{tabular}{l|cccc|cccc}
\hline
\multirow{2}{*}{Configuration} & \multicolumn{4}{c|}{Fuzzy Clustering Metrics} & \multicolumn{4}{c}{Rule Violations} \\
& FPC & FPE & MS & FS & Stealth & UAV & Mission & Semantic \\
\hline
Baseline & 0.5401 & 0.9775 & 0.396 & -- & -- & -- & -- & -- \\
2-Rule & 0.9765 & 0.0474 & 0.9850 & -- & 85 & 214 & -- & -- \\
4-Rule & 0.4736 & 1.1456 & 0.6184 & 0.1960 & 85 & 90 & 533 & 0 \\
\hline
\multicolumn{9}{l}{\footnotesize FPC: Fuzzy Partition Coefficient, FPE: Fuzzy Partition Entropy,} \\
\multicolumn{9}{l}{\footnotesize MS: Average Membership Strength, FS: Fuzzy Silhouette Index}
\end{tabular}
\end{table*}

